Strong coloring numbers of grids

For positive integers $n$ and $d$, the $d$-dimensional grid of side length $n$ is the graph $G(n,d)$ with vertex set $[n]^d$, in which two vertices are adjacent if they differ by $1$ in exactly one coordinate and agree in all the other coordinates. We determine, for every fixed $d$, the asymptotic growth in $r$ of the $r$th strong coloring numbers of these grids. More precisely for $n$ large enough, ${\rm scol}_r(G(n,d)) = \Omega_d\bigl(r^{d-1}\bigr)$ as $r\to\infty$. This matches an upper bound given by a volume packing argument, which holds more generally for touching graphs of unit balls in $\mathbb R^d$. For the lower bound, we construct in $G(n,d)$ a bramble of order $\Omega_d(n^{d-1})$ with each element of radius at most $dn$. This construction was found by OpenAI's GPT-5.6 Sol.

==> style.toc.tex <==
% https://tex.stackexchange.com/questions/633286/how-to-add-dots-to-ams-table-of-contents
\usepackage{xpatch}
\makeatletter   
\xpatchcmd{\@tocline}
{\hfil\hbox to\@pnumwidth{\@tocpagenum{#7}}\par}
{\ifnum#1<2\hfill\else\dotfill\fi\hbox to\@pnumwidth{\@tocpagenum{#7}}\par}
{}{}
\makeatother    
% *******************************************   

\makeatletter
\def\l@section{\bfseries\@tocline{1}{0pt}{0pc}{4pc}{}}
\def\l@subsection{\mdseries\@tocline{2}{0pt}{4pc}{6pc}{}}
\def\l@subsubsection{\mdseries\@tocline{3}{0pt}{8pc}{8pc}{}}
\makeatother

\renewcommand\contentsname{\vspace{-1cm}}
